Using Deep Learning to Solve Computer Security Challenges: A Survey

Although using machine learning techniques to solve computer security challenges is not a new idea, the rapidly emerging Deep Learning technology has recently triggered a substantial amount of interests in the computer security community. This paper seeks to provide a dedicated review of the very recent research works on using Deep Learning techniques to solve computer security challenges. In particular, the review covers eight computer security problems being solved by applications of Deep Learning: security-oriented program analysis, defending return-oriented programming (ROP) attacks, achieving control-flow integrity (CFI), defending network attacks, malware classification, system-event-based anomaly detection, memory forensics, and fuzzing for software security.

==> Makefile <==
default: testfornewtable

PAPER = testfornewtable
SCRIPT = manuscript
REFERENCE = aisecsurvey
JUNK =*.log *.synctex\(busy\) *.xml *.bcf *.toc *.snm *.nav *.fls *.fdb_latexmk *.synctex.gz *.spl *.ps *.dvi  *.out *.aux *.backup *~ *.blg *.bbl
COUNTING_TOOL = ./texcount.pl
TEMP = 0
MY_VAR=$(shell echo whatever)

# Define the tools we are going to use

# Rules for various parts of the target
testfornewtable: $(PAPER).tex
	pdflatex $(PAPER).tex
	bibtex $(PAPER).aux
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex
	rm -f $(JUNK)

manuscript: $(SCRIPT).tex
	pdflatex $(SCRIPT).tex
	bibtex $(SCRIPT).aux
	pdflatex $(SCRIPT).tex
	pdflatex $(SCRIPT).tex
	rm -f $(JUNK)

clean:
	rm -f $(JUNK) $(PAPER).pdf

counting: 
	./texcount.pl -merge canary.tex

counting-detail: 
	./texcount.pl -inc canary.tex
	 


==> sections/panalysis/table.tex <==

\begin{table}[!h]
    \begin{threeparttable}
  % h, here
  % t, top
  % b, bottom
  % p, page of float
    \caption{Comparison of phase3 in different works.}
    \label{tab:comp}
  % \makeatletter
  % \newcommand{\widenhline}{%
  %     \noalign {\ifnum 0=`}\fi \hrule height 0.5pt
  %     \futurelet \reserved@a \@xhline
  % }
  % \newcolumntype{I}{!{\vrule width 1pt}}
  % \makeatother
  \centering
  \small
  \begin{tabular}{p{2.5cm}||c p{3.5cm} c c p{2cm} c}  
  \hline  
  \hline  
  Paper  &  Considertaion &  Motivation~\tnote{1} & Adoption & Explanation~\tnote{2}  & Validation~\tnote{3} & Comparison~\tnote{4}\\ 
  \hline  
  Function Identification~\cite{shin2015recognizing} & \ding{51}  & They believe that the attractive features of neural networks is that they can learn directly from the original representation with minimal preprocessing. 
            &  \ding{55} &   N/A           & N/A                           & N/A\\ 
  
  \hline  
  EKLAVYA~\cite{chua2017neural} & \ding{51}   & To enhance model's ability of generalization.  
            &  \ding{51}   &  \ding{51}      & t-SNE \& Analogical reasoning & \ding{51}\\ 
  \hline  
  Gemini~\cite{xu2017neural}  & \ding{51}   & Transfer Graph to Vector.  
            &  \ding{51} &     \ding{55}       & N/A                           & \ding{55} \\ 
  \hline  
  DEEPVSA~\cite{guo2019deepvsa} & \ding{51}      & Learn the dependency within instructions.
            &  \ding{51} & \ding{51}  & Empirical method & \ding{51}\\ 
  
  \hline 
  \hline   
  \end{tabular} 
      \begin{tablenotes}
          \item[1] The reason for their adoption of representative learning.
          \item[2] Explaining the representative learning.
          \item[3] Methods used for validate the effect of representative learning.
          \item[4] Comparison with other representative learning methods.
      \end{tablenotes}
  \end{threeparttable}
  \end{table}
